ArctyrEX : Accelerated Encrypted Execution of General-Purpose Applications

Fully Homomorphic Encryption (FHE) is a cryptographic method that guarantees the privacy and security of user data during computation. FHE algorithms can perform unlimited arithmetic computations directly on encrypted data without decrypting it. Thus, even when processed by untrusted systems, confidential data is never exposed. In this work, we develop new techniques for accelerated encrypted execution and demonstrate the significant performance advantages of our approach. Our current focus is the Fully Homomorphic Encryption over the Torus (CGGI) scheme, which is a current state-of-the-art method for evaluating arbitrary functions in the encrypted domain. CGGI represents a computation as a graph of homomorphic logic gates and each individual bit of the plaintext is transformed into a polynomial in the encrypted domain. Arithmetic on such data becomes very expensive: operations on bits become operations on entire polynomials. Therefore, evaluating even relatively simple nonlinear functions, such as a sigmoid, can take thousands of seconds on a single CPU thread. Using our novel framework for end-to-end accelerated encrypted execution called ArctyrEX, developers with no knowledge of complex FHE libraries can simply describe their computation as a C program that is evaluated over $40\times$ faster on an NVIDIA DGX A100 and $6\times$ faster with a single A100 relative to a 256-threaded CPU baseline.

==> figures/blas_topology_2.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{images/blas_topology_2.png}
    \caption{\textbf{Topology of Matrix Benchmarks}: both benchmarks exhibit ample parallelism, with matrix multiplication being consistently twice as wide for most levels.}\label{f:blas_topology_2}
\end{figure}


==> figures/dispatch.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\columnwidth]{NDSS-2024/images/arctyrex-dispatch.png}
    \caption{\textbf{Dispatch System}: a coordinator computes \st{shares} \fixsd{shards ?!?} of each level of a Boolean netlist and distributes these workloads to CPU workers. For systems with GPUs, each worker is connected to a dedicated GPU.}\label{f:dispatch}
\end{figure}


==> figures/dispatch_algo.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{$circuit$, $numWorkers$}
Allocate memory for intermediate data \linebreak
(I) Perform breadth-first search to determine widest level \linebreak
(II) Allocate enough memory to store $maxWires \times ctxtSize$ elements\\
$workQueues = new Queue[numWorkers]$\\
\For{level in circuit}{
    $cnt = 0$ \\
    \For{gate in level}{
        $workQueues[cnt \mathbin{\%} numWorkers].append(gate)$ \linebreak
        $cnt += 1$
    } 
    Signal workers to begin evaluation \\
    Block until all workers finish
}\KwRet
 \caption{Runtime Library Dispatch Algorithm \fixca{Update to reflect current implementation if possible}\fixca{Cedric: rewrite!}}
 \label{alg:dispatch}
\end{algorithm}

==> figures/dispatch_algo_new.tex <==
%\begin{algorithm}
%\SetAlgoLined
%\KwIn{$levels$, $numWorkers$}
%$nsteps = batched_waves.size()$\\
%\For {$wave$ in $batched\_waves$}
%{
%    \For {$batch_id$ in $wave.size()$}
%    {
%        // Dispatch GPU batches accross GPUs
%        int dev_id = batch_id % numWorkers;
%        process_batch(&batches[batch_id], dev_id);
%    }
%
%    bool need_sync = (step == nsteps - 1);\\
%    fence_on_devices(need_sync);\\
%}
% \caption{\textcolor{black}{Runtime Library Dispatch Algorithm}}
% \label{alg:dispatch}
%\end{algorithm}
\begin{lstlisting}

int dev_id = 0;
for (auto &wave : batched_waves)
{
    for (auto &batch : wave)
        process_batch(&batches[batch_id],
                      (dev_id++)%nWorkers);

    fence();
}
\end{lstlisting}

==> figures/gemm_code.tex <==
\newsavebox{\mm}
\begin{lrbox}{\mm}
\begin{lstlisting}[language=C,
    breaklines=true,         
    basicstyle=\ttfamily\footnotesize,
    numbers=left,
    numberstyle=\scriptsize\color{gray},
    keywordstyle=\color{blue},
    commentstyle=\itshape\color{gray}
]
void full_gemm(short x[100], short y[100], short res[100]) {
  for (int i = 0; i < 10; i++) {
    for (int j = 0; j < 10; j++) {
      res[10*i + j] = 0;
      for (int k = 0; k < 10; k++) {
        res[10*i + j] = res[10*i + j] + x[i*10 + k] * y[k*10 + j];
      }
    }
  }
  return;
}
\end{lstlisting}
\end{lrbox}

\begin{figure}[ht!]
\centering
\usebox{\mm}
\caption{Full Matrix Multiplication HLS Kernel}\label{f:mm}
\end{figure}


==> figures/logic-gate.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.6\columnwidth]{images/cggi-gate.png}
    \caption{\textbf{Encrypted Logic Gate Evaluation}: all standard two-input logic gates begin with a series of linear operations between the input LWE ciphertexts, followed by a bootstrapping procedure (executed by the looped instructions), and lastly a keyswitching operation.}\label{f:logic_gate}
\end{figure}

==> figures/ml_nn_topology.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{NDSS-2024/images/fhedinn_topology.png}
    \caption{\textbf{FHE-DiNN Neural Network Topology}: The plaintext weight variant exhibits a shorter critical path and is composed of much fewer gates overall.}\label{f:ml_nn_topology}
\end{figure}


==> figures/preprocess_algo.tex <==
\begin{algorithm}
\SetAlgoLined
\KwIn{$circuit, numWorkers$}
\KwOut{$levels$}
$levels = $ new $Queue[circuit.depth()]$\\
$readyQueue = $ new $Queue$\\
$pending = $ new $HashMap<Gate, int>$\\
$step = 1$\\
$maxGates = 0$\\

\For{gate in circuit}{
    $pending[gate] = gate.numOperands$ \\
    \If{$gate.numOperands == 0$}{
        $readyQueue.append(gate)$\\
        $levels[0].append(gate)$
    }
}

\While{$readyQueue$ is not empty}{
    \If{$readyQueue.size() > maxGates$}{
        $maxGates = readyQueue.size()$
    }
    $nextReadyQueue = $ new $Queue$\\
    \While{$readyQueue$ is not empty}{
        $Gate$ $ n = readyQueue.front()$\\
        $readyQueue.pop()$
        \For{$gate$ in n.operands}{
            $pending[gate] = pending[gate] - 1$\\
            \If{$pending[gate] == 0$}{
                $nextReadyQueue.append(gate)$
            }
        }
    }
    \While{$nextReadyQueue$ is not empty}{
        $Gate$ $ n = nextReadyQueue.front()$\\
        $nextReadyQueue.pop()$\\
        $readyQueue.append(n)$\\
        $levels[step].append(n)$
    }
    $step = step + 1$
}
$maxMemory = maxGates * 2 * sizeof(Ctxt)$\\
 Allocate $maxMemory$ bytes\\
\KwRet
 \caption{\textcolor{black}{Runtime Library Circuit Preprocessing}}
 \label{alg:preprocess}
\end{algorithm}

==> figures/tikz_dispatch.tex <==
\definecolor{myyellow}{HTML}{FFD965}

\begin{figure}[!ht]
\centering
\begin{tikzpicture}
    [
        dot/.style = {fill=myyellow, text=red, shape=circle, minimum size=100pt, inner sep=2pt},
        rectext/.style= {rectangle, minimum width=2.85cm, minimum height=1cm, align=center, text width=2.95cm, font=\small,
        fill=myyellow}
    ]
\begin{scope}[transform shape, scale=0.5]
\draw
node[dot, font=\Large](0){Coordinator}
node[auto=false, below=4.5cm of 0, font=\Huge](dots){\dots}
node[auto=false, below=1.75cm of dots](comm_text){Ciphertext Communication}

node[inner sep=0pt, left=0.75cm of dots] (gpu1){
\includegraphics[width=.165\textwidth,trim={0 0 27cm 0cm},clip]{NDSS-2024/figures/gpu_arch.jpg}
}
node[inner sep=0pt, left=0.5cm of gpu1] (gpu2){
\includegraphics[width=.165\textwidth,trim={0 0 27cm 0cm},clip]{NDSS-2024/figures/gpu_arch.jpg}
}
node[inner sep=0pt, left=0.5cm of gpu2]{GPUs}

node[inner sep=0pt, right=0.75cm of dots] (gpuN){
\includegraphics[width=.165\textwidth,trim={0 0 27cm 0cm},clip]{NDSS-2024/figures/gpu_arch.jpg}
}
node[inner sep=0pt, right=0.5cm of gpuN] (gpuN1){
\includegraphics[width=.165\textwidth,trim={0 0 27cm 0cm},clip]{NDSS-2024/figures/gpu_arch.jpg}
}
;

% \draw [stealth-stealth, dashed](0) -- (Worker1);
% \draw [stealth-stealth, dashed](0) -- (Worker2);
% \draw [stealth-stealth, dashed](0) -- (WorkerN) node[left, midway]{Batch${_N}$};
% \draw [stealth-stealth, dashed](0) -- (WorkerNand1);

\draw [stealth-stealth](gpu1) -- (0);
\draw [stealth-stealth](gpu2) -- (0);
\draw [stealth-stealth](gpuN) -- (0) node[left, midway, text width=1.25cm]{Kernel Launch};
\draw [stealth-stealth](gpuN1) -- (0);

\draw 
[dashed](gpu1.south) -- ++(0,-1) node[](A){}
-| node(B){} (gpu2)
[dashed](B) -| node(C){} node[above, pos=0.25]{} (gpuN)
[dashed](C) -| (gpuN1);

\end{scope}

\end{tikzpicture}

    \caption{\textbf{Dispatch System}: A coordinator computes batches of each level of a Boolean netlist and distributes these workloads to GPU workers.}\label{f:dispatch}
    \fixcg{Cedric: I am unsure this picture is really useful ...}
\end{figure}

==> figures/tikz_overview.tex <==
\definecolor{myblue}{HTML}{BDD7EE}

\begin{figure}[!ht]
\centering
\begin{tikzpicture}
    [
        dot/.style = {fill, shape=circle, minimum size=5pt, inner sep=0pt},
        rectext/.style= {rectangle, minimum width=2.85cm, minimum height=1cm, align=center, text width=2.95cm, font=\small,
        fill=myblue}
    ]

\begin{scope}[transform shape, scale=0.90]
\draw
node[rectext](0){C/C\texttt{++} Program}
node[rectext, right=2.25cm of 0](1){Multi-Bit\\ Arithmetic Circuit}
node[rectext, right=2.25cm of 1](2){Boolean Netlist}
node[draw, dashed, rectangle, rounded corners, minimum height=2cm, minimum width=15cm](box1) at (1){}
node[above=0.01mm of 1](a){Frontend}
;

\draw [-stealth](0.east) -- (1.west) node[above, midway, font=\scriptsize]{HLS};
\draw [-stealth](1.east) -- (2.west) node[above, midway, font=\scriptsize]{Logic Synthesis} node[below, midway, font=\scriptsize]{Circuit Optimizations};

\draw
node[rectext, below=1.5cm of 2](3){Planning and Mem Allocation}
node[rectext, left=2.25cm of 3](4){Coordinator Thread}
node[rectext, left=2.25cm of 4](5){Workers}
node[draw, dashed, rectangle, rounded corners, minimum height=2.5cm, minimum width=15cm] at (4){}
node[above=0.01mm of 4](b){Middle-Layer(Runtime Library)}
;

\draw [-stealth](2.south) -- (3.north) node[]{};
\draw [-stealth](3.west) -- (4.east) node[above, midway, font=\scriptsize]{};
\draw [stealth-stealth](4.west) -- (5.east) node[above, midway, font=\scriptsize]{Batch Assignment} node[below, midway, font=\scriptsize]{Status};

\draw
node[rectext, below=2.25cm of 5](6){GPU 0}
node[rectext, right=2.25cm of 6](7){Crypto\\Implementation\\\hfill\\\scriptsize{Fused Kernels/\\Optimized Data Transfers}}
node[rectext, right=2.25cm of 7](8){Math Primitives\\\hfill\\\scriptsize{NTT\\Modular Arithmetic}}
node[draw, dashed, rectangle, rounded corners, minimum height=3.5cm, minimum width=15cm] at (7){}
node[above=0.01mm of 7](b){Back-End (CUDA CGGI)}
;

\draw [-stealth](5.south) -- (6.north) node[]{};
\draw [dotted](6.east) -- (7.west) node[above, midway, font=\scriptsize]{};
\draw [-stealth](7.east) -- (8.west) node[above, midway, font=\scriptsize]{};
\end{scope}

\end{tikzpicture}

    \caption{\textbf{System Overview:} The proposed system is composed of three distinct layers that work together to realize an end-to-end framework for encrypted computation. The frontend converts high-level programs to a logic circuit tuned for FHE. In turn, this logic circuit is parsed by the middle layer, which incorporates a coordinator thread that partitions each level of the circuit into shares which are assigned to an arbitrary number of worker threads. Lastly, the back-end is utilized by each worker thread to outsource computationally expensive FHE operations to a dedicated GPU.}\label{f:overview}
\end{figure}

